SpheRoPE: Zero-Shot Optimization-Free 360 Panorama Generation with Spherical RoPE

We present a zero-shot, training-free and optimization-free framework for generating 360 panoramic images and videos by directly injecting spherical priors into pre-trained diffusion transformers. Existing methods either rely on costly fine-tuning on scarce panoramic data that limits generalization, or leverage multi-step optimization that incurs prohibitive inference latency. We observe that contemporary generative models natively exhibit some panoramic priors from large-scale training. However, these emergent capabilities are insufficient, as the models fundamentally fail to satisfy the rigorous topological constraints imposed by equirectangular projection (ERP). We introduce a zero-shot and optimization-free approach that resolves these constraints at inference time. Spherical RoPE replaces standard rotary position embeddings: low-frequency channels are re-parameterized as 3D Cartesian coordinates to natively encode the spherical manifold, while high-frequency channels are harmonically quantized to enforce exact periodicity. Coupled with complementary Semantic Distortion classifier-free guidance (CFG) that explicitly steers geometry, we avoid retraining and inherit the full creative breadth of state-of-the-art models. Our approach generalizes across diverse backbones and 360 generation modalities. We demonstrate this across text-to-panorama using Flux.1, Flux.2, and LTX-Video backbones, achieving competitive performance against baselines, all while remaining training-free. Project page: https://orhir.github.io/SpheRoPE

==> tables/FID_50_prompts.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{4pt}
\caption{\textbf{Quantitative comparison on 50 diverse prompts outside the training distribution of prior indoor-focused methods.} 
We report image-based metrics computed against ImageNet statistics, including FID/KID variants and Inception Score (IS), along with CLIP Score (CS) and Discontinuity Score (DS). 
KID is reported as $\times 10^{-2}$.  
Best results are shown in \textbf{bold} and second-best are \underline{underlined}.}
\label{tab:inet_metrics}
\scriptsize
\begin{tabular}{lccccccccccc}
\toprule
Method 
& inet-FID $\downarrow$ 
& inet-crop-FID $\downarrow$ 
& inet-mv-FID $\downarrow$ 
& inet-KID $\downarrow$ 
& inet-crop-KID $\downarrow$ 
& inet-mv-KID $\downarrow$ 
& IS $\uparrow$ 
& crop-IS $\uparrow$ 
& mv-IS $\uparrow$ 
& CS $\uparrow$ 
& DS $\downarrow$ \\
\midrule

PanFusion 
& \underline{300.22} 
& \underline{157.64} 
& 201.36 
& \underline{9.25} 
& 4.97 
& 6.11 
& 2.72 
& 6.96 
& 5.73 
& \underline{30.76} 
& \underline{1.0610} \\

UniPano 
& 340.84 
& 159.95 
& \textbf{198.56} 
& 12.99 
& \textbf{4.18} 
& \textbf{4.02} 
& \underline{2.82} 
& \textbf{8.54} 
& \textbf{7.39} 
& 29.26 
& 1.1502 \\

SpheRoPE 
& \textbf{293.06} 
& \textbf{150.24} 
& \underline{198.99} 
& \textbf{8.16} 
& \underline{4.48} 
& \underline{5.13} 
& \textbf{2.89} 
& \underline{7.80} 
& \underline{7.09} 
& \textbf{31.68} 
& \textbf{0.8792} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/FID_table.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{4pt}
\caption{\textbf{Quantitative comparison across panorama and multi-view settings.} 
All metrics are computed on Matterport3D~\cite{chang2017matterport3d}. 
We evaluate panoramas using FAED, FID, IS, CLIP Score (CS), and \textbf{Discontinuity Score (DS)}~\cite{christensen2024geometry}. 
Following prior work~\cite{tang2023mvdiffusion, zhang2024panfusion}, we sample 20 random views and 8 horizontal views. 
\textit{inet-FID} denotes FID computed against ImageNet statistics. 
\textbf{SphereRoPe*} employs LLM-based prompt rewriting to produce semantically equivalent but more descriptive inputs aligned with the expectations of Flux2 (Claude Opus 4.6; prompt provided in the Supplementary). }
\label{tab:panorama_results}
\scriptsize
\begin{tabular}{lcccccc|ccc|cccc}
\toprule
& \multicolumn{6}{c|}{Panorama} 
& \multicolumn{3}{c|}{20 Views} 
& \multicolumn{4}{c}{Horizontal 8 Views} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-10} \cmidrule(lr){11-14}
Method 
& FAED $\downarrow$ & FID $\downarrow$ & inet-FID $\downarrow$ & IS $\uparrow$ & CS $\uparrow$ & DS $\downarrow$
& FID $\downarrow$ & inet-FID $\downarrow$ & IS $\uparrow$
& FID $\downarrow$ & inet-FID $\downarrow$ & IS $\uparrow$ & CS $\uparrow$ \\
\midrule


PanFusion 
& \textbf{5.69} & 47.08 & 190.60 & 4.31 & 28.62 & 0.73
& 17.66 & \textbf{121.10} & 7.04
& 20.17 & 124.10 & 6.72 & 24.98 \\

UniPano 
& 7.62 & \textbf{44.69} & 194.60 & 3.89 & 28.37 & 0.76
& \textbf{16.76} & 123.20 & 6.65
& \textbf{17.67} & 128.55 & 5.90 & 24.93 \\

\textbf{SphereRoPe} 
& 39.15 & 85.03 & 192.92 & 4.47 & 28.76 & \textbf{0.64}
& 42.05 & 124.38 & 6.97
& 43.75 & 144.18 & 6.09 & 24.74 \\

\textbf{SphereRoPe*} 
& \textbf{18.93} & 85.25 & \textbf{182.86} & \textbf{4.60} & \textbf{29.20} & 0.80
& 54.36 & 123.65 & \textbf{8.00}
& 48.39 & \textbf{108.85} & \textbf{8.25} & \textbf{27.49} \\

\bottomrule
\end{tabular}
\end{table*}

==> tables/ablation_flux1.tex <==
   \begin{table}[t]
   \centering
   \caption{\textbf{Components Contribution (FLUX.1).} We ablate key components of our method: spherical RoPE and ERP-aware CFG.
   Best in \textbf{bold}, second best \underline{underlined}.}
   \label{tab:ablation_flux1}
   \resizebox{\columnwidth}{!}{%
   \begin{tabular}{l|cc|ccc}
   & \multicolumn{2}{c|}{\textbf{Panorama-Level Metrics}} & \multicolumn{3}{c}{\textbf{Perspective Crop Metrics}} \\
   \textbf{Configuration} & OmniFID $\downarrow$ & DS $\downarrow$ & FID $\downarrow$ & KID$_{\times 10^2}$ $\downarrow$ & IS $\uparrow$ \\
   \midrule
   % Vanilla FLUX.1 & 106.85 & 12.10 & 37.62 & \underline{1.49} & \underline{10.88} \\
   % Vanilla FLUX.1(360 prefix) & 90.33 & 8.64 & 29.39 & 1.05 & 11.26 \\
   \textbf{Full method} & \textbf{85.67} & \textbf{0.89} & \underline{35.02} & \underline{1.56} & \underline{10.69} \\
   \quad w/o spherical RoPE & 94.92 & 1.42 & 42.31 & 2.14 & 9.93 \\
   \quad w/o Semantic Distortion CFG & \underline{104.34} & \underline{1.02} & \textbf{34.25} & \textbf{1.27} & \textbf{11.69} \\
   \bottomrule
   \end{tabular}%
   }
   \end{table}

==> tables/quantitative_v2.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Quantitative comparison}. We compare our zero-shot results with training-based methods on the ODISR dataset. 
We show both panorama-level metrics and multi-view metrics (computed from 8 equally spaced horizontal perspective crops). \sagie{will adding inference speed column be in our favor?} 
% Cells are colored per column from \colorbox[rgb]{0,1,0.15}{green} (best) to \colorbox[rgb]{1,0,0.15}{red} (worst). 
Best in \textbf{bold}, second best \underline{underlined}.}
\label{tab:quantitative}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|ccc|cccc}
\toprule
& & \multicolumn{3}{c|}{\textbf{Panorama-Level Metrics}} & \multicolumn{4}{c}{\textbf{Multi-View Metrics}} \\
\textbf{Method} & \textbf{Type} & FAED $\downarrow$ & OmniFID $\downarrow$ & DS $\downarrow$ & FID $\downarrow$ & KID$_{\times 10^2}$ $\downarrow$ & IS $\uparrow$ & CS $\uparrow$ \\
\midrule
Text2Light~\cite{chen2022text2light} & Full Fine-Tune & \cellcolor[rgb]{0.91,0.73,0.73}77.94 & \cellcolor[rgb]{0.91,0.73,0.73}121.90 & \cellcolor[rgb]{0.91,0.73,0.73}3.87 & \cellcolor[rgb]{0.91,0.73,0.73}81.01 & \cellcolor[rgb]{0.91,0.73,0.73}4.55 & \cellcolor[rgb]{0.91,0.75,0.73}6.25 & \cellcolor[rgb]{0.73,0.91,0.73}\textbf{18.60} \\
Diffusion360~\cite{feng2023diffusion360} & Full Fine-Tune & \cellcolor[rgb]{0.91,0.78,0.73}71.02 & \cellcolor[rgb]{0.90,0.91,0.73}96.17 & \cellcolor[rgb]{0.78,0.91,0.73}0.87 & \cellcolor[rgb]{0.91,0.90,0.73}53.17 & \cellcolor[rgb]{0.91,0.90,0.73}2.82 & \cellcolor[rgb]{0.91,0.89,0.73}8.92 & \cellcolor[rgb]{0.76,0.91,0.73}18.46 \\
StitchDiffusion~\cite{wang2024stitchdiffusion} & LoRA & \cellcolor[rgb]{0.91,0.83,0.73}63.10 & \cellcolor[rgb]{0.91,0.89,0.73}100.78 & \cellcolor[rgb]{0.85,0.91,0.73}1.01 & \cellcolor[rgb]{0.86,0.91,0.73}43.73 & \cellcolor[rgb]{0.83,0.91,0.73}1.84 & \cellcolor[rgb]{0.83,0.91,0.73}10.88 & \cellcolor[rgb]{0.75,0.91,0.73}18.50 \\
PanFusion~\cite{zhang2024panfusion} & LoRA & \cellcolor[rgb]{0.83,0.91,0.73}39.29 & \cellcolor[rgb]{0.87,0.91,0.73}92.39 & \cellcolor[rgb]{0.86,0.91,0.73}1.09 & \cellcolor[rgb]{0.84,0.91,0.73}40.37 & \cellcolor[rgb]{0.86,0.91,0.73}2.12 & \cellcolor[rgb]{0.90,0.91,0.73}9.66 & \cellcolor[rgb]{0.91,0.80,0.73}17.14 \\
UnoPano~\cite{ni2025makes} & LoRA & \cellcolor[rgb]{0.87,0.91,0.73}46.19 & \cellcolor[rgb]{0.91,0.91,0.73}97.55 & \cellcolor[rgb]{0.87,0.91,0.73}1.10 & \cellcolor[rgb]{0.80,0.91,0.73}34.76 & \cellcolor[rgb]{0.82,0.91,0.73}1.78 & \cellcolor[rgb]{0.89,0.91,0.73}9.73 & \cellcolor[rgb]{0.91,0.73,0.73}16.81 \\
SMGD~\cite{sun2025smgd} & Full Fine-Tune & \cellcolor[rgb]{0.79,0.91,0.73}33.55 & \cellcolor[rgb]{0.89,0.91,0.73}94.91 & \cellcolor[rgb]{0.75,0.91,0.73}\underline{0.80} & \cellcolor[rgb]{0.89,0.91,0.73}49.02 & \cellcolor[rgb]{0.85,0.91,0.73}2.01 & \cellcolor[rgb]{0.91,0.73,0.73}5.77 & \cellcolor[rgb]{0.75,0.91,0.73}18.52 \\
DiT360~\cite{feng2025dit360} & LoRA & \cellcolor[rgb]{0.86,0.91,0.73}43.42 & \cellcolor[rgb]{0.73,0.91,0.73}\textbf{73.72} & \cellcolor[rgb]{0.91,0.80,0.73}2.15 & \cellcolor[rgb]{0.73,0.91,0.73}\textbf{23.28} & \cellcolor[rgb]{0.74,0.91,0.73}0.92 & \cellcolor[rgb]{0.73,0.91,0.73}\textbf{12.90} & \cellcolor[rgb]{0.75,0.91,0.73}\underline{18.52} \\
PAR~\cite{wang2025conditional} & Full Fine-Tune & \cellcolor[rgb]{0.80,0.91,0.73}34.79 & \cellcolor[rgb]{0.84,0.91,0.73}88.67 & \cellcolor[rgb]{0.73,0.91,0.73}\textbf{0.76} & \cellcolor[rgb]{0.75,0.91,0.73}25.80 & \cellcolor[rgb]{0.73,0.91,0.73}\textbf{0.85} & \cellcolor[rgb]{0.86,0.91,0.73}10.47 & \cellcolor[rgb]{0.75,0.91,0.73}18.51 \\
\midrule
Ours (FLUX.1) & \textbf{Zero-Shot} & \cellcolor[rgb]{0.76,0.91,0.73}\underline{29.94} & \cellcolor[rgb]{0.88,0.91,0.73}93.99 & \cellcolor[rgb]{0.79,0.91,0.73}0.89 & \cellcolor[rgb]{0.87,0.91,0.73}45.22 & \cellcolor[rgb]{0.91,0.91,0.73}2.63 & \cellcolor[rgb]{0.86,0.91,0.73}10.32 & \cellcolor[rgb]{0.75,0.91,0.73}18.52 \\
\textbf{Ours (FLUX.2)} & \textbf{Zero-Shot} & \cellcolor[rgb]{0.73,0.91,0.73}\textbf{25.40} & \cellcolor[rgb]{0.81,0.91,0.73}\underline{83.52} & \cellcolor[rgb]{0.80,0.91,0.73}0.91 & \cellcolor[rgb]{0.75,0.91,0.73}\underline{25.33} & \cellcolor[rgb]{0.74,0.91,0.73}\underline{0.90} & \cellcolor[rgb]{0.74,0.91,0.73}\underline{12.75} & \cellcolor[rgb]{0.77,0.91,0.73}18.43 \\
\bottomrule
\end{tabular}%
}
\end{table*}


==> tables/vbench.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{3.5pt}
\caption{\textbf{VBench comparison~\cite{vbench2024}.}
Subject/Background Consistency measure temporal stability of appearance (subject via DINO features, background via CLIP features), distinct from Motion Smoothness (movement continuity).
Temporal Flickering measures frame coherence (higher = less flicker), Imaging Quality measures perceptual quality, and CLIP Mean measures text--video alignment.
Higher is better ($\uparrow$). Best in \textbf{bold}, second-best underlined.}
\label{tab:vbench}
\scriptsize
\begin{tabular}{lcccccc}
\toprule
\textbf{Method}
& \shortstack{\textbf{Imaging}\\\textbf{Quality} $\uparrow$}
& \shortstack{\textbf{CLIP}\\\textbf{Mean} $\uparrow$}
& \shortstack{\textbf{Temporal}\\\textbf{Flickering} $\uparrow$}
& \shortstack{\textbf{Motion}\\\textbf{Smoothness} $\uparrow$}
& \shortstack{\textbf{Subject}\\\textbf{Consistency} $\uparrow$}
& \shortstack{\textbf{Background}\\\textbf{Consistency} $\uparrow$} \\
\midrule
DynamicScaler~\cite{liu2025dynamicscaler}
& \underline{0.5353} & \underline{27.4548} & 0.9711 & 0.9810 & 0.9380 & 0.9473 \\
360DVD~\cite{wang2024360dvd}
& 0.4442 & 25.6066 & 0.9781 & 0.9851 & 0.9377 & 0.9475 \\
SphereDiff~\cite{park2025spherediff}
& 0.4008 & 26.5465 & \underline{0.9935} & \underline{0.9951} & \underline{0.9590} & \underline{0.9633} \\
Ours
& \textbf{0.5364} & \textbf{27.5695} & \textbf{0.9958} & \textbf{0.9962} & \textbf{0.9822} & \textbf{0.9771} \\
\bottomrule
\end{tabular}
\end{table*}
